Collective excitations of a strongly-correlated non-equilibrium photon fluid across the Mott/superfluid phase transition

We develop a Gutzwiller theory for the non-equilibrium steady states of a strongly-interacting photon fluid driven by a non-Markovian incoherent pump. In particular, we explore the collective excitation modes across the out-of-equilibrium Mott/superfluid transition, characterizing the diffusive Goldstone mode in the superfluid phase and the particle/hole excitations in the insulating one. Observable features in the pump-and-probe optical response of the system are highlighted. Our results appear as experimentally accessible to state-of-the-art circuit-QED devices and open the way for driven-dissipative fluids of light as quantum simulators of novel many-body scenarios.

==> 100_words.tex <==
We develop a Gutzwiller theory for the collective excitations of a strongly-correlated driven-dissipative photon fluid under non-Markovian pumping, which displays a non-equilibrium instance of the Mott/superfluid phase transition. We specifically characterize the particle/hole and diffusive Goldstone modes on the insulating and superfluid sides of the transition, and anticipate their observable signatures in the dynamical response of the system to additional weak probe beams. Our work provides guidance for the understanding and design of experiments on fluids of light in state-of-the-art circuit-QED systems, and a novel theoretical tool for the investigation of exotic states of matter emerging in driven-dissipative lattice models.
% We expect that our work will provide a guidance for experiments on fluids of light in state-of-the-art circuit-QED systems, as well as a novel theoretical tool for the investigation of exotic states of matter that emerge in driven-dissipative lattice models.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> work_file.tex <==



==> work_file_SM.tex <==


